D-CIPHER: Dynamic Collaborative Intelligent Multi-Agent System with Planner and Heterogeneous Executors for Offensive Security

Large Language Models (LLMs) have been used in cybersecurity such as autonomous security analysis or penetration testing. Capture the Flag (CTF) challenges serve as benchmarks to assess automated task-planning abilities of LLM agents for cybersecurity. Early attempts to apply LLMs for solving CTF challenges used single-agent systems, where feedback was restricted to a single reasoning-action loop. This approach was inadequate for complex CTF tasks. Inspired by real-world CTF competitions, where teams of experts collaborate, we introduce the D-CIPHER LLM multi-agent framework for collaborative CTF solving. D-CIPHER integrates agents with distinct roles with dynamic feedback loops to enhance reasoning on complex tasks. It introduces the Planner-Executor agent system, consisting of a Planner agent for overall problem-solving along with multiple heterogeneous Executor agents for individual tasks, facilitating efficient allocation of responsibilities among the agents. Additionally, D-CIPHER incorporates an Auto-prompter agent to improve problem-solving by auto-generating a highly relevant initial prompt. We evaluate D-CIPHER on multiple CTF benchmarks and LLM models via comprehensive studies to highlight the impact of our enhancements. Additionally, we manually map the CTFs in NYU CTF Bench to MITRE ATT&CK techniques that apply for a comprehensive evaluation of D-CIPHER's offensive security capability. D-CIPHER achieves state-of-the-art performance on three benchmarks: 22.0% on NYU CTF Bench, 22.5% on Cybench, and 44.0% on HackTheBox, which is 2.5% to 8.5% better than previous work. D-CIPHER solves 65% more ATT&CK techniques compared to previous work, demonstrating stronger offensive capability.

==> tables/categorywise_results.tex <==
\begin{table}[htpb]
    \centering
    \footnotesize
    
    \begin{tabular}{lcccccc}
    \toprule
    & cry. & foren. & pwn & rev & web & misc \\
    \cmidrule(lr){2-7}
    \multicolumn{7}{l}{\textbf{NYU CTF baseline}}\\
    \smalltab Claude & 7.7 & \textbf{20.0} & 7.7 & 21.6 & 5.3 & 16.7 \\
    \smalltab GPT 4o & 3.8 & 0.0 & 5.1 & 9.8 & 0.0 & 12.5 \\
    \smalltab GPT 4T. & 1.9 & 0.0 & 5.1 & 9.8 & 0.0 & 16.7 \\
    \multicolumn{7}{l}{\textbf{EnIGMA}}  \\
    \smalltab Claude & 7.7 & \textbf{20.0} & 18.0 & 17.7  & 0.0 & 16.7 \\
    \smalltab GPT 4o & 3.9 & 13.3 & 7.7 & 13.7 & 5.3 & 16.7 \\
    \smalltab GPT 4T. & 1.9 & 13.3 & 5.1 & 9.8 & 0.0 & 16.7 \\
    \multicolumn{7}{l}{\textbf{D-CIPHER}}  \\
    \smalltab Claude & \textbf{15.4} & \textbf{20.0} & 12.8 & \textbf{29.4} & 5.3 & \textbf{25.0} \\
    \smalltab GPT 4o & 5.8 & 13.3 & 7.7 & 13.7 & \textbf{10.5} & 16.7 \\
    \smalltab GPT 4T. & 1.9 & 13.3 & 5.1 & 7.8 & 5.3 & 12.5 \\
    \smalltab LLaMa & 1.9 & 0.0 & 0.0 & 3.9 & 0.0 & 12.5 \\
    \smalltab Gemini & 1.9 & 0.0 & 0.0 & 3.9 & 0.0 & 8.3 \\
    \multicolumn{7}{l}{\textbf{D-CIPHER} w/o auto-prompter}\\
    \smalltab Claude & \textbf{15.4} & \textbf{20.0} & \textbf{28.2} & 27.5 & \textbf{10.5} & \textbf{25.0} \\
    \smalltab GPT 4o & 1.9 &	6.7 &	5.1 &	17.6 &	10.5 &	16.7 \\
    \multicolumn{7}{l}{\textbf{D-CIPHER} w/o planner}\\
    \smalltab Claude & 9.6 &	6.7 &	7.7 &	25.5 &	5.3 &	20.8  \\
    \smalltab GPT 4o & 3.8	& 6.7 & 	5.1 &	13.7 &	5.3 &	20.8  \\
    \bottomrule
    \end{tabular}
    \caption{\emph{\% solved} by category on NYU CTF Bench of D-CIPHER and related works.}
    \label{tab:categorywise}
\end{table}
